Unveiling the main sequence of galaxies at $z \geq 5$ with the James Webb Space Telescope: predictions from simulations

We use two independent, galaxy formation simulations, FLARES, a cosmological hydrodynamical simulation, and SHARK, a semi-analytic model, to explore how well the James Webb Space Telescope (JWST) will be able to uncover the existence and parameters of the star-forming main sequence (SFS) at $z=5\to10$, i.e. shape, scatter, normalisation. Using two independent simulations allows us to isolate predictions (e.g., stellar mass, star formation rate, SFR, luminosity functions) that are robust to or highly dependent on the implementation of the physics of galaxy formation. Both simulations predict that JWST can observe $\ge 70-90\%$ (for SHARK and FLARES respectively) of galaxies up to $z\sim10$ (down to stellar masses of $\approx 10^{8.3}\,\rm M_{\odot}$ and SFRs of $\approx 10^{0.5}\,\rm M_{\odot}\, yr^{-1}$) in modest integration times and given current proposed survey areas (e.g. the Web COSMOS $0.6\,\rm deg^2$) to accurately constrain the parameters of the SFS. Although both simulations predict qualitatively similar distributions of stellar mass and SFR, there are important quantitative differences, such as the abundance of massive, star-forming galaxies, with FLARES predicting a higher abundance than SHARK; the early onset of quenching as a result of black hole growth in FLARES (at $z\approx 8$), not seen in SHARK until much lower redshifts; and the implementation of synthetic photometry, with FLARES predicting more JWST-detected galaxies ($\sim 90\%$) than SHARK ($\sim 70\%$) at $z=10$. JWST observations will distinguish between these models, leading to a significant improvement upon our understanding of the formation of the very first galaxies.

==> Sections/spare.tex <==
“Figure 11 shows the ratio of total flux of galaxies that are fainter than 29 magnitudes to total flux of galaxies in Flares and Shark. We calculate this by integrating the light functions predicted by the simulations. We investigate the flux ratio observed in the F775W filter of the Advanced Camera for Surveys of the HST, the motivation for which is that this filter was used for source detection to the same limiting magnitude of ∼ 29 mag in the Hubble Ultra Deep Field (Beckwith et al. 2006a), and the F200W filter of NIRCam of the JWST. The purpose of this figure is two fold. We show this result only for galaxies with M★ ≥ 108.5M⊙ , which we expect to be star forming as per the SFS. 
 
First, we see that the differences in the dust attenuation prescription between the two simulations affects the fraction of Hubble-dark galaxies. At �� ≳ 8 both simulations predict that almost all galaxies will be undetected by the HST as a result of the rest-wavelengths becoming more so affected by dust attenuation. For 6 ≲ �� ≲ 8, Flares predicts ∼ 100% Hubble-dark galaxies compared to Shark where the fraction reduces from ∼ 100% at �� = 8 to a few percent at �� = 6. The fraction is greater in Flares at these redshifts because the normalisation of the SFRs allows for dustier galaxies. At �� ∼ 5, however the fraction of Hubble-dark galaxies (a few percent) in Shark is greater than that of Flares (almost zero percent), despite Flares having a higher normalisation of the SFRF. This is where the instantaneous chemical enrichment in Shark becomes apparent and produces more obscured systems with the same star formation rate than Flares. Overall, it is a combination of both the star formation prescription and dust attenuation that produces a significant population of Hubble-dark galaxies at �� ≳ 5.  
 
The second purpose of this plot is to show that the F200W filter of NIRCam on the JWST is far less affected by the dust than the HST. We see that there are virtually no JWST-dark galaxies in Flares at all redshifts, while the fraction systematically decreases from ∼ 10% at �� = 10 to a few tenths of a percent at �� = 5 in Shark. Therefore, there will still be a population of undetected JWST galaxies in Shark; although, not significant enough to hinder a parametrisation of the SFS as we detailed in Section 4. Ultimately, this shows that JWST, with continued observations, will be able to distinguish differences in the dust modelling of galaxies of independent simulations.” 


\begin{figure*}
    \centering
    \includegraphics[width = \linewidth]{Figures/galaxies-fraction.pdf}
    \caption{The ratio of number of faint galaxies (>29 mag, top) and bright galaxies (<29 mag, bottom) in a given filter to total number of galaxies. Solid lines show the results for the F775W filter of the Advanced Camera for Surveys on the HST, and dashed lines show the results for the F200W filter of NIRCam on the JWST. Left panels show the results for a stellar mass cut of $\mathrm{M_{\star}\geq 10^{8.3}M_{\odot}}$, and right panels show the results for a SFR cut of $\mathrm{SFR \geq 10^{0}M_{\odot}yr^{-1}}$. Orange lines show results for \textsc{Flares} and blue lines show results for \textsc{Shark}.}
    \label{fig:flux_fraction}
\end{figure*}

{ \bf The effect of dust on the number of observed galaxies can be seen in \Cref{fig:flux_fraction}, which shows the ratio of the number of galaxies that are fainter than 29 magnitudes to total number of galaxies in \textsc{Flares} and \textsc{Shark}. We investigate this ratio for galaxies observed in the F775W filter of the Advanced Camera for Surveys of the HST - which is the filter used for source detection in the Hubble Ultra Deep Field \citep{beckwithHubbleUltraDeep2006a} - and the F200W filter of NIRCam of the JWST.

We see in the top and bottom panels that HST-dark galaxies are significant at all redshifts, going from $\sim 100\%$ at $z=10$ to $\lesssim 1\%$ at $z=5$ in \textsc{Flares}, and $\sim 100\%$ at $z=10$ to $\sim 20\%$ at $z=5$ in \textsc{Shark}. This is true for both stellar mass and SFR cuts investigated. 
%We see that the HST-dark fraction is smaller in \textsc{Flares} at $z=5$ at fixed SFR ($\sim 0.1\%$) instead of fixed stellar mass ($\0.4\%$), whereas the fraction remains the same in \textsc{Shark}. 
This is related to the instantaneous chemical enrichment in \textsc{Shark} that produces dustier systems than \textsc{Flares} for a fixed SFR, the effect of which becomes increasingly more important in the lead up to the peak of cosmic star formation rate density at $z\sim2$. 

We see that both simulations predict a population of JWST-dark galaxies, going from $\sim 10\%$ at $z=10$ to $\lesssim 1\%$ at $z=5$ in \textsc{Flares}, and $\sim 30\%$ at $z=10$ to $\sim 3\%$ at $z=5$ in \textsc{Shark}. Though the fraction of missing galaxies due to dust obscuration is not significant enough to hinder a thorough exploration of the $\mathrm{SFR-M_{\star}}$ and is far less with JWST at $z=5\to10$ compared to HST. The fact that these fractions are varied between the simulations boils down to different prescriptions of stellar mass assembly and dust attenuation. The JWST should be able to detect sufficiently many galaxies to distinguish between these model dependent prescriptions.}









\subsection{Dust attenuation differences}

%\Cref{fig:f200w_z6-10} shows that the proportion of galaxies that the JWST will be able to observe is model dependent. As 
We have established that the two simulations model the assembly of stellar mass similarly; however, the differences in the treatment of dust and attenuation in the simulations yields quite different predictions of the number of galaxies that are currently observable by HST (Fig.~\ref{fig:fuv_z6-10}).  
%is the greater delineator between \textsc{Flares} and \textsc{Shark}. The ability for the JWST to comprehend these differences will serve to improve the understanding and implications of dust between $\mathrm{z = 5\to 10}$, particular upon the galactic sources of reionisation highlighted in the bottom row of \Cref{fig:fuv_z6-10}. The build up of dust in those high redshift galaxies is thus connected with the formation of the first galaxies. 

\begin{figure*}
    \includegraphics[width=\textwidth]{Figures/att_hexplots_z6_to_z10.png}
    \caption{$\mathrm{SFR-M_{\star}}$ at redshifts ${z=6,8,10}$ for \textsc{Flares} (above) and \textsc{Shark} (below). We discretised the plane into hexagonal bins of equal area, and colour them according to the median FUV attenuation in each. Each bin contains a minimum of 5 objects. The scale is shown in the colour bar on the right. Points indicate single galaxies with the same colour scheme indicating their attenuation. The grey shaded regions show the approximate stellar mass resolution limit of $\mathrm{10^{8.5}M_{\odot}}$.}
    \label{fig:att_hexplots}
\end{figure*}

\Cref{fig:att_hexplots} shows the median $A_{\rm FUV}$ of galaxies in the $\mathrm{SFR-M_{\star}}$ plane at ${z=6,8,10}$ for \textsc{Flares} (top) and \textsc{Shark} (bottom),  where the FUV attenuation is calculated as
\begin{equation}
    \mathrm{A_{FUV} = -2.5 \log_{10}(FUV_{obsc}/FUV_{intr}).}
    \label{eq:fuv_att}
\end{equation}
\noindent Here, $\mathrm{FUV_{obsc}}$ is the FUV flux observed through the dusty medium and $\mathrm{FUV_{intr}}$ is the FUV flux before it has been attenuated by dust. It can be seen that in both simulations there exists a population of highly attenuated systems toward the top-end of the $\mathrm{SFR-M_{\star}}$ at all redshift. 

Broadly, the attenuation in both simulations traces the SFS, with dustier galaxies inhabiting the top end of it, $\mathrm{M_{\star}\gtrsim10^{9}M_{\odot}}$. {\bf However, the attenuation gradient tracks more closely with stellar mass in \textsc{Flares}, whereas it tracks more so with SFR in \textsc{Shark}, for all redshifts shown here.}
% {\bf There are more attenuated systems at fixed high SFR (e.g., $\mathrm{SFR \sim 10^{0.5} M_{\odot}yr^{-1}}$ at $z=6$) in \textsc{Shark} than in \textsc{Flares}.}
% In addition, {\sc Shark} yields higher values of  $A_{\rm FUV}$ for the most star-forming and massive galaxies in the simulation, compared to {\sc Flares}. 
This is related to to the instantaneous chemical enrichment model adopted in {\sc Shark} which allows very starbursting galaxies to enrich their ISM with metals very quickly compared to {\sc Flares}, where a delay is applied. {\bf We also inspected the gas phase metallicities in the simulations and found that \textsc{Shark} predicted higher metallicities per unit stellar mass and SFR at $z=5$ and $z=10$ than \textsc{Flares}.} This corroborates the differences in the CSMH and CSFRH between the two simulations that was discussed in \cref{sect:cosmic}. Because both simulations use the gas mass in metals as proxies for the dust content of galaxies, it is clear that the chemical enrichment model plays a critical role in the predicted dust attenuation. 


%This is strong evidence that instantaneous enrichment is somewhat responsible for the differences in the cosmic histories. In fact, the higher specific SFR over most stellar masses and most redshifts in \textsc{Flares} compared to \textsc{Shark} also agrees with this. 
%An objective of the JWST will be to try and distinguish between these two models so that the connection between dust and star formation can more easily be unveiled. As both simulations connect dust with the gas metallicity it implies that the JWST should be well poised to investigate the transition between metal free and metal rich star formation in the early universe. 

%{\bf A related result} is the difference between the normalisation of the CSFRH for the total population of either simulation being greater than that of the CSMH, with \textsc{Shark} predicting a lower normalisation than \textsc{Flares} for both quantities at all redshifts shown. The reason for this disparity is the method of chemical enrichment used in each. For an episode of star formation \textsc{Shark} instantaneously diverts mass from stars to metals in the interstellar medium \citep{Lagos2018}, while there is a delay between star formation and enrichment in \textsc{Flares} to account for the evolution of supernovae and AGB stars \citep{Crain_2015,Schaye2015}. This, in combination with the excess stellar mass and SFR number density, explain this difference in the cosmic histories.

% \begin{figure*}
%     \includegraphics[width=\textwidth]{Figures/fuv_band7_distributions.pdf}
%     \caption{Intrinsic FUV (left column) and obscured ALMA band-7 (right column) LFs at redshifts $\mathrm{z=6,8}$ (as labelled) for \textsc{Flares} (top four panels) and \textsc{Shark} (bottom four panels) for galaxies with $\mathrm{M_{\star}\geq 10^{9}M_{\odot}}$. The black dashed lines show the quantities for the entire population in the simulations. The red lines show the quantities for the JWST detected populations, the blue lines show the quantities for the HST detected populations and the yellow lines show the quantities for the $\mathrm{HST \cup JWST}$ populations. The orange and blue dotted lines show the FUV distributions for the entire population of all stellar masses in \textsc{Flares} and \textsc{Shark}, respectively.}
%     \label{fig:band7_fuv}
% \end{figure*}

% The current lack of infrared and sub-mm observations beyond $\mathrm{z \sim 2}$ have made it difficult to constrain the amount of obscured SFR and stellar mass. \citet{Casey_2018} explain this with two dust paradigms that exist beyond $\mathrm{z \sim 2}$: one where the proportion of dusty galaxies is negligible and one where the bulk of cosmic SFR is contributed by dusty galaxies, both of which are able to explain the lack of CSFRH as derived from short wavelength surveys. \citet{Casey_2018} conclude that it is not yet possible with current instruments to distinguish between the two with high redshift constraints from the IR and sub-mm, although recent observations tend to prefer a dust-poor early Universe (e.g. \citealt{Casey21,Zavala21}).  
% %%With such a census of high redshift galaxies, each of the models presented in \citet{Casey_2018} can be tested by follow up observations across the breadth of the electromagnetic spectrum. 


% \Cref{fig:band7_fuv} shows the redshift $\mathrm{z=6,8}$ intrinsic FUV  ($\sim1500$\AA) and ALMA band-7 ($\sim 8.5 \mu$m) number densities for galaxies detectable by the JWST, by the HST and by either the JWST or the HST in \textsc{Flares} and \textsc{Shark}. The radiative transfer 
% %ACA VOY
% analysis code SKIRT \citep{Camps2018} was used to analyse the FIR emission of only those FLARES galaxies that contained $\ge 1000$ star particles, which translates to a stellar mass threshold of $\mathrm{\sim 10^{9}M_{\odot}}$ \citep{vijayan2021light}. Thus, we show these results for galaxies above this stellar mass in both \textsc{Flares} and \textsc{Shark}. SKIRT was also used to produce the FUV emission, which is an entirely different attenuation model than that of \citet{Vijayan2021}, which is what we use in the previous FUV results presented in this paper; we do not show the SKIRT derived FUV distributions in this figure. The line-of-sight attenuation model of \textsc{Flares}, which is used in the majority of this work, is simpler than the full SKIRT model to enable feasible computation but fails to model particular phenomena like scattering away from the line of sight or dust self absorption since both of these are reliant on the chosen extinction curve. The line-of-sight model was found to predict magnitude distributions that are systematically shifted $\mathrm{\sim 0.4 dex}$ fainter than those derived with the SKIRT model. The dust optical depth along the line of sight in the line-of-sight model was found to be lower than in the SKIRT model. For a deeper discussion of the differences the reader is refered to \citet{vijayan2021light}. 

% We show the distributions that the JWST, HST and JWST or HST will be able to recover, and compare these to the total distribution above the stellar mass threshold. HST detected galaxies are considered to be those with $\mathrm{app \, mag \leq 29 \,AB \,mag}$ when viewed through the F775W filter ($0.75\mu$m) of the HST Advance Camera for Surveys (ACS). Beyond $\mathrm{z=8}$ we predict that there are very few galaxies above $\mathrm{M_{\star}\sim 10^{9}M_{\odot}}$. The take home message here is that the HST is unable to survey enough galaxies needed to constrain FUV and sub-mm fluxes during the epoch of reionisation. The ACS is largely unable to provide sufficient galaxy samples needed to perform follow up observations in the sub-mm with ALMA. 
% %%This alludes to the latter of the dust scenarios in \citep{Casey_2018} as the HST detected populations are a fraction of the total population indicating that the majority of galaxies are obscured by dust. 
% From the right column in \Cref{fig:band7_fuv} we see that the JWST detected ALMA band-7 distribution is very similar to the total population up to at least $\mathrm{z=8}$. This is important as the galaxy census provided by the JWST will be subject to ALMA follow up observations meaning that ALMA will be able to quantify the sub-mm emission for representative galaxies in the Universe during the epoch of reionisation. We note that the band-7 distributions are very model dependent, with \textsc{Shark} typically predicting brighter dust emission by $2$ orders of magnitude compared to \textsc{Flares}. \citet{lovell2021simba} used the \textsc{Simba} simulation suite \citep{dave2019simba} to show that ability to reproduce sub-mm counts in simulations was most reliant on the normalisation of the star formation rate function. Thus, it is interesting that we see such disagreement in the sub-mm emission between \textsc{Shark} and \textsc{Flares} despite the broad agreement in their respective star formation rate functions. Therefore, we conclude that the difference is driven by the differences in the dust enrichment and emission mechanisms in the simulations, particularly the instantaneous enrichment in \textsc{Shark} that allows for much brighter sub-mm emission. 

%We have shown that the JWST will be able to detect sufficiently many galaxies to determine the distributions of stellar mass and star formation to $\mathrm{z=10}$. 

% \subsection{The volume probed by JWST surveys}

% So far we have not accounted for the survey volume required to ascertain a sample representative of the Universe. Uncertainties in pencil beam surveys such as the Hubble Ultra Deep Field \citep{Beckwith2006} are dominated by cosmic variance where the probability of obtaining a survey sample representative of the entire Universe scales with area coverage \citep{DriverRobotham2010}. 

% \begin{figure}
%     \includegraphics[width=\linewidth]{Figures/volume-comparison.pdf}
%     \caption{Evolution of the area covered by the box size of the simulation volumes, \textsc{Flares} in orange and \textsc{Shark} in blue. The light grey and dark grey dotted lines shows the area coverage of the Hubble COSMOS survey \citep{Scoville2007} and Webb COSMOS survey \citep{kartaltepe2021} respectively.} 
%     \label{fig:volume_comp}
% \end{figure}

% \Cref{fig:volume_comp} shows the redshift evolution of the area covered by the simulation volumes in reference to the area covered by the Hubble \citep{Scoville2007} and Webb \citep{kartaltepe2021} COSMOS programs, which cover $\mathrm{\sim2.0\, deg^{2}}$ and $\mathrm{\sim0.7 \, deg^{2}}$, respectively. It should be noted that we only include the cumulative volume of the $40$ zoom regions sampled in \textsc{Flares}. As \textsc{Flares} samples regions of a range of overdensities from a larger $\mathrm{3.2^{3}\,Gpc^{3}}$ DM-only simulation the coverage shown in \Cref{fig:volume_comp} is likely a lower limit, with the maximum limit being the area covered by the larger DM-only box; but we do not show this here. \textsc{Flares} covers a smaller area than that of the largest proposed JWST survey of $\mathrm{\sim0.7 \, deg^{2}}$ implying that Webb COSMOS will be able to observe a similar number of galaxies contained in \textsc{Flares}. \textsc{Shark} covers more area than Webb COSMOS implying that this survey will likely not be able to observe the same number of galaxies in \textsc{Shark}. 

% The fact that the area covered by \textsc{Shark} and \textsc{Flares} simulated boxes are either greater than the largest proposed survey with the JWST or a lower limit of the possible probed volume has implications on our ability to constrain the parameters of the SFS, as this relies on a sufficiently well sampled $\mathrm{SFR-M_{\star}}$. To account for this effect we refit the SFS, using the same methods in \Cref{sect:SFS}, for the JWST detected population but halve the number of galaxies used in the fitting. 

% \begin{figure*}
%     \includegraphics[width=\textwidth]{Figures/resample_sfs.pdf}
%     \caption{\textit{Top four panels:} Redshift evolution of the parameters of the SFS. The dashed orange and blue lines with shaded regions show the results and 1$\sigma$ uncertainties for the JWST detected population in \textsc{Flares} and \textsc{Shark} respectively. The red and cyan lines with error bars show the results and 1-$\sigma$ uncertainties for half of the JWST detected population in \textsc{Flares} and \textsc{Shark} respectively. Each fit uses a 0.2 and 0.4 dex Gaussian uncertainty on $\mathrm{M_{\star}}$ and $\mathrm{SFR}$ respectively. \textit{Bottom two panels: } $\mathrm{SFR-M_{\star}}$ at $\mathrm{z=6}$ and $\mathrm{z=10}$ as labelled. The grey shaded region shows approximate stellar mass resolution limit of $\mathrm{10^{8.5}M_{\odot}}$. The dotted lines with shaded regions show the median and 5-95 quantiles for the total galaxy population in \textsc{Flares} (orange) and \textsc{Shark} (blue). The orange and blue dashed lines show the fitted SFS for the JWST detected population for \textsc{Flares} and \textsc{Shark} respectively. The solid red and cyan lines show the fitted SFS for one half of the JWST detected galaxies for \textsc{Flares} and \textsc{Shark} respectively. These lines are virtually identical.} 
%     \label{fig:resampled}
% \end{figure*}

% \Cref{fig:resampled} shows the results of this exercise. We see that even when we only use half of the JWST detected galaxies, with a $0.2$ and $0.4$~dex Gaussian uncertainty on $\mathrm{M_{\star}}$ and $\mathrm{SFR}$ respectively, we can still recover the parameters of the SFS of the underlying galaxies in both simulations.
% %for the net JWST detected population, which is related to the total, true, population by \Cref{fig:sfs_jwst_fit}, within uncertainties for all redshifts between $\mathrm{z=5\to10}$. 
% This provides an indication as to how the coverage of surveys affects constraints on the SFS; the key result being that even with at least half the approximate survey area of the simulations, acknowledging the caveats inherent in \textsc{Flares}, JWST should still be able to constraints on the SFS. 
% %Still, even half the areas covered by the simulations will likely be larger than the largest proposed JWST survey, the Webb COSMOS survey at the time of writing, meaning that wide JWST surveys are necessary for future studies on the SFS.

% \begin{figure}
%     \includegraphics[width=\linewidth]{Figures/expected.pdf}
%     \caption{Differential stellar mass (top) and SFR (bottom) number counts for \textsc{Flares} (left) and \textsc{Shark} (right) at $\mathrm{z=6, 8, 10}$ (colours) as labelled. We assume a redshift separation of $\mathrm{\Delta z = 1}$ and an area coverage of $\mathrm{\Delta \Omega = 1 \, deg^{2}}$. The shaded regions in all panels highlight where there is less than one object per bin.}
%     \label{fig:expected}
% \end{figure}

% \Cref{fig:expected} shows the expected differential stellar mass and SFR counts for the JWST detected galaxies in \textsc{Flares} and \textsc{Shark} at $\mathrm{z=6,8,10}$. The calculation is
% \begin{equation}
%     \mathrm{dN_{exp}/dX = \phi(X) \frac{dV}{dzd\Omega}\Delta z \Delta \Omega},
%     \label{eq:expected}
% \end{equation}

% \noindent where $\mathrm{\phi(X)}$ are the number densities of \Cref{fig:smf_sfrf_z6-10}, $\mathrm{\frac{dV}{dzd\Omega}}$ is the differential comoving volume, $\mathrm{\Delta z = 1}$ is the redshift separation and $\mathrm{\Delta \Omega = 1 \, deg^{2}}$ is the survey area. This is similar to the expected number counts presented in \citet{Shen2021}, who used the {\sc Illustris-TNG} simulation to predict JWST luminosity functions. Even at $\mathrm{z=10}$ we will be able to recover a few $\mathrm{M_{\star}\sim10^{10}M_{\odot}}$ galaxies and their SFRs. This suggests that the $\mathrm{SFR-M_{\star}}$ can be explored with current planned surveys with the JWST, though wider surveys would be of great benefit to thoroughly study the intricacies of the SFS during the epoch of reionisation. 
 % \cref{fig:volume} shows the area that corresponds to the simulation volume at $\mathrm{z=5\to10}$. We show the area of the underlying $\mathrm{3.2\,Gpc^{3}}$ dark matter only simulations from which \textsc{Flares} samples and the area obtained from the 40 of $\mathrm{14 h^{-1}\,Mpc}$ \textsc{Flares} zoom volumes. The `effective' volume of \textsc{Flares} is considered to lie somewhere between these two. We show the area coverage of the COSMOS HST survey \citep{Scoville2007} that covers $\mathrm{1.8deg^{2}}$ and the proposed coverage of COSMOS-Webb \citep{kartaltepe2021} that will cover $\mathrm{0.6deg^{2}}$
%JWST distributions being different --> dust treatment --> sfs hex plots = dust + sfr + mstar assembly => transition from metal free to metallic star formation --> casey dust paradigms/ jwst detect all bright galaxies --> follow ups




% Talk about HST observations and how they are obscured and thus need to be corrected.

% Need to talk about how JWST will be able to decouple differences in the simulations. Connect attenuation with SFS show hex plots




\caption{\textit{Top: } Averaged $\mathrm{\chi^{2}}$ values for each of the SFS fits where we have resampled galaxy stellar masses and SFRs according to different survey volumes 10 times for \textsc{Flares} (left) and \textsc{Shark} (right). $\mathrm{\chi^{2} = \sum^{4}_{i=0}\frac{(x_{i}-x^{true}_{i})^{2}}{x^{true}_{i}}}$ where $\mathrm{x_{i}}$ represents the derived parameters of the resampled SFS and $\mathrm{x_{i}^{true}}$ the derived parameters for the entire population in the simulations. Filled circles show the  $\mathrm{\chi^{2}}$ for the JWST-detected galaxies; upright, left-pointing and right-pointing triangles show the $\mathrm{\chi^{2}}$ for a JWST surveys of areas $\mathrm{220arcmin^{2}}$ (i.e. a single pointing), $\mathrm{220arcmin^{2}}$ (i.e. a medium deep field) and $\mathrm{0.6deg^{2}}$ (i.e. the Web COSMOS survey), respectively, as labelled. \textit{Bottom: } SFS plots at ${z=5}$ (left) and ${z=10}$ (right), for \textsc{Flares} (red and orange colours) and \textsc{Shark} (blue and cyan colours). We use the same symbols and colour gradient as the top panels to reflect different fits for each sample. Orange and blue shaded regions show the $5^{\rm th}-95^{\rm th}$ percentile ranges for all galaxies in the simulations.}
